sketch-plot: Progressive Editing for Text-to-Image Academic Figures

Text to image (T2I) models such as gpt-image-2 can now generate publication grade academic figures from a short prompt, but the output is a flat raster: a user who wants to change one arrow, one label, or one icon has to regenerate the whole image, which also disturbs the parts they wanted to keep. We present sketch-plot, an interactive system that closes this controllability gap with a three layer progressive editing pipeline: a generated PNG, an addressable puzzle of editable pieces, and a per piece SVG. The user stops at the layer that gives them enough control for the change at hand, so the cost of decomposition and vectorisation is paid only on the pieces that need it. Realising this pipeline is not trivial. General segmentation models lack the semantic discriminability to decompose a research figure cleanly, and end to end image vectorisation produces incomplete shapes and loses semantic structure. We therefore route both stages through a human in the loop interface that lets the user accept, refine, or reject decomposition and vectorisation decisions on a piece by piece basis. We validate the design with an expert user study, in which participants found sketch-plot effective for making targeted edits to AI generated academic figures and preferred it over regenerating the whole image. A demonstration video is available at https://paper-plot.dev/sketch.

==> sec/benchmark.tex <==
\section{Benchmark}
\label{sec:benchmark}

To systematically evaluate the quality of generated interactive documents, we construct \textsc{ViviBench}, a benchmark consisting of a curated topic dataset grounded in real-world interactive documents and an automated evaluation framework covering four complementary dimensions.

\subsection{Dataset}
\label{sec:dataset}

A key challenge in benchmarking interactive document generation is obtaining topics that reflect genuine needs rather than synthetic or contrived examples.
To address this, we adopt a reverse-engineering approach: we collect 101 real-world interactive documents from 63 distinct websites across 11 subject areas, including platforms such as \texttt{setosa.io}~\cite{setosa} and \texttt{distill.pub}~\cite{hohman2020communicating}.      
For each document, we use an LLM to extract the core topic as a concise natural-language description (e.g., ``Exponential growth as repeated multiplication'').
These extracted topics serve as the input prompts for all generation methods.
Due to space limitations, we provide the distribution of topics across subject areas in the supplementary material.

From these 101 documents, we also extract 482 interaction instances. Three visualization experts collaboratively classify these instances into 8 interaction types based on interaction intent such as Parameter Exploration and State Switching (see Figure \ref{fig:cases}). This taxonomy inspires the design of the SRTC Interaction Specification (Section~\ref{sec:spec}), which can express all 8 identified types.

% \begin{table}[t]
%   \caption{Distribution of topics in \textsc{ViviBench} by subject area.}
%   \label{tab:dataset}
%   \begin{tabular}{lr}
%     \toprule
%     Subject Area & \# Topics \\
%     \midrule
%     Algorithms & 25 \\
%     Mathematics & 24 \\
%     Tools \& Resources & 13 \\
%     Physics & 10 \\
%     Science & 9 \\
%     Other & 6 \\
%     Explorable Explanations & 5 \\
%     Systems \& Thought Experiments & 4 \\
%     Psychology & 2 \\
%     Creativity & 2 \\
%     Books \& Essays & 1 \\
%     \midrule
%     \textbf{Total} & \textbf{101} \\
%     \bottomrule
%   \end{tabular}
% \end{table}

\begin{figure*}[t]
  \centering
  \includegraphics[width=0.85\textwidth]{image/system.pdf}
  \caption{The \system user interface. Top: the main view with (A) sidebar for history and new document creation, (B) center panel with topic input and four-stage navigation bar, and (C) AI chat assistant. Bottom (left to right): the Spec stage showing editable knowledge units, the Style stage with writing and interaction style options, and the Doc stage displaying the generated interactive document.}
  \label{fig:system}
\end{figure*}

\subsection{Evaluation Metric}
\label{sec:evaluation}

We evaluate generated documents along four dimensions using a two-layer evaluation framework. The first layer applies deterministic, rule-based checks to verify functional correctness and generation efficiency. The second layer employs LLM-as-Judge to assess higher-level content and interaction quality~\cite{zheng2023judging, xie2025visjudge}.

\paragraph{Layer 1: Rule-based Evaluation.}
Two dimensions are evaluated through automated checks, providing reproducible and deterministic assessments:

\begin{itemize}[nosep,leftmargin=*]
  \item \textbf{Interaction Functionality (IF):} Tests whether interactive elements (buttons, sliders, checkboxes, dropdowns) respond to programmatic interaction using Playwright browser automation. For each element, we record the DOM state before and after triggering the interaction; elements that produce a DOM change are counted as functional. The score is the ratio of responsive elements to total interactive elements found.
  \item \textbf{Efficiency (Eff):} Measures the generation throughput as the ratio of output HTML length (in characters) to generation time (in seconds). This metric captures how efficiently each method utilizes its LLM calls to produce content.
\end{itemize}

\paragraph{Layer 2: LLM-as-Judge Evaluation.}
Two dimensions are assessed by prompting an LLM to score each document on a 1--5 Likert scale with detailed rubrics:

\begin{itemize}[nosep,leftmargin=*]
  \item \textbf{Content Richness (CR):} Whether the document covers the topic with sufficient breadth (e.g., multiple sub-concepts) and depth (e.g., explanations, examples, connections between ideas). We extract the main textual content from the HTML, stripping scripts and styling, so the judge focuses on the educational substance rather than code volume.
  \item \textbf{Interaction Quality (IQ):} A composite metric defined as $\text{IQ} = \text{ID} \times \text{IF}$, where ID (Interaction Design) is the LLM-judged score for whether interactive elements serve a clear purpose, and IF is the rule-based Interaction Functionality score. This formulation ensures that only functionally working interactions contribute to the quality score.
\end{itemize}


==> sec/demo.tex <==
\section{Demo Walkthrough}
\label{sec:demo}

We show \system on two scenarios drawn from real authoring tasks.

\subsection{Adjusting a generated teaser figure}

A user generates a teaser figure from the prompt ``a poster for an interactive document research project: three example cards in the middle row, four skill icons at the bottom, hand drawn aesthetic''. The L1 raster contains six high level units: a title block, an author row, three example image cards, four skill cards, a separator, and a footer CTA. Clicking \emph{Shatter} runs L2: \texttt{gemini-3.1-pro-preview} returns the layout JSON in about 9 seconds, and the partition completion pass adds three background fragments for the gaps. The user notices that the title bounding box is too narrow on the right (the VLM clipped the title at character 24 of an actual 48 character title). They grab the shared edge between the title and the right margin fragment, and drag it 200 px to the right. Both pieces update in lockstep; the right margin fragment is promoted from \texttt{background} to \texttt{fragment 1}. The user then runs L3 on the title piece, which produces an SVG containing the full text as a single editable string. They fix a typo by editing the SVG directly and copy the result to a slide deck.

\subsection{Localised edit on a pipeline diagram}

A user uploads an existing pipeline figure showing three panels labelled (a)~Overall Pipeline, (b)~How an Evaluator Agent is Configured, (c)~What is Evaluated. They want to swap the trophy icon in panel (a) for a checklist icon. They click panel (a) to select it, type ``replace the trophy icon with a clipboard icon, keep all other elements identical'' into the side panel, and click \emph{Apply edit}. The system crops panel (a)'s bounding box from the source raster, sends \texttt{(crop, prompt)} to the inpaint endpoint, and re composites the returned crop into the original image. The other two panels are untouched at the pixel level, which is the controllability property that full image regeneration cannot offer.

\subsection{Interaction primitives}

Table~\ref{tab:prims} lists the puzzle paradigm's interaction vocabulary as exposed by \system. Each primitive is defined identically on named pieces and on background fragments, per principle (P2).

\begin{table}[h]
    \caption{Interaction primitives, defined uniformly over named pieces and background fragments.}
    \label{tab:prims}
    \small
    \begin{tabular}{ll}
        \toprule
        Primitive & Effect \\
        \midrule
        Hover     & Show label and copy/tray buttons \\
        Click     & Open side inspector \\
        \texttt{Cmd+C}  & Copy piece PNG to clipboard \\
        \texttt{+ tray} & Stash piece in bottom tray \\
        Drag edge & Resize the two adjacent pieces in lockstep \\
        Apply edit & Inpaint piece with user prompt \\
        To SVG    & Run L3 vectorisation on this piece \\
        \bottomrule
    \end{tabular}
\end{table}


==> sec/spec.tex <==
\section{Document Specification}
\label{sec:spec}

The Document Specification (DocSpec) is the structured intermediate representation at the core of \system. It bridges the gap between a high-level topic and the generated interactive document by decomposing the content into a sequence of knowledge units, each with explicit instructions for both text and interaction generation.

\subsection{Structure}

A DocSpec consists of a topic and an ordered list of knowledge units. Each knowledge unit contains three components:

\begin{itemize}[noitemsep,leftmargin=10pt]
    \item A \textbf{unit summary} that briefly states the concept covered.
    \item A \textbf{text description} that provides a self-contained guide for generating the explanatory text of the section. It specifies what the reader should understand after reading, without prescribing exact wording.
    \item An \textbf{Interaction Specification} that defines the interactive visualization using the SRTC decomposition described below.
\end{itemize}

The text description and Interaction Specification serve different steps of the Executor: the former guides Step 1 (text generation) and the latter guides Step 2 (visualization generation). This separation allows each step to operate independently with minimal ambiguity. The Interaction Specification supports all common interaction patterns such as parameter exploration, direct manipulation, and mode switching (see Figure \ref{fig:cases}). Due to space limitations, we provide the corresponding specifications for these cases in the supplementary material.

\subsection{Interaction Specification: SRTC}

Munzner's What-Why-How framework~\cite{munzner2014visualization} provides a foundational decomposition for visualization design: What data is being visualized, How it is visually encoded and interacted with, and Why the user engages with it. We adapt this framework to the setting of LLM-based generation by introducing the SRTC Interaction Specification, which decomposes each interactive visualization into four components:

\begin{itemize}[noitemsep,leftmargin=10pt]
    \item \textbf{State (S)}: The variables underlying the visualization, including their types, domains, default values, and derivation rules. Variables are either user-controllable (e.g., a slider with a specified range) or derived from other variables (e.g., a formula). This corresponds to Munzner's What.
    \item \textbf{Render (R)}: A description of how the state maps to visual elements on screen, such as geometric shapes, labels, or charts. This corresponds to the visual encoding aspect of How.
    \item \textbf{Transition (T)}: A description of how user actions modify the state, specifying the cause-and-effect relationship between input events and state changes. This corresponds to the interaction idiom aspect of How.
    \item \textbf{Constraint (C)}: The key invariant that the visualization is designed to demonstrate. This is the core insight the reader should discover through interaction. This corresponds to Munzner's Why, adapted from ``what task is the user performing'' to ``what should the reader observe.''
\end{itemize}

\paragraph{Example.} Table~\ref{tab:spec-example} contrasts a natural language interaction description with its corresponding SRTC specification for a visualization about $\pi$. The natural language version leaves implicit what variables exist, how they relate, what appears on screen, and what invariant the reader should notice. The SRTC version makes each of these explicit. The State defines a user-controllable variable $r$ (a slider over $[0.5, 5]$) and three derived variables: circumference $C = 2\pi r$, diameter $D = 2r$, and their ratio $C/D$. The Render specifies that the visualization displays a circle whose size reflects $r$, along with labels for $C$, $D$, and the ratio. The Transition links the slider interaction to the state: dragging the slider changes $r$, and all derived variables update automatically. Finally, the Constraint encodes the key invariant that the reader should discover: $C/D \approx 3.14159$ regardless of $r$.

\begin{table}[t]
  \caption{Comparison of a natural language interaction description and its SRTC Interaction Specification for a visualization about $\pi$.}
  \label{tab:spec-example}
  \small
  \centering
  \begin{tabularx}{\columnwidth}{@{}lX@{}}
\toprule
\multicolumn{2}{@{}l}{\textbf{Natural language description}} \\
\midrule
\multicolumn{2}{@{}p{\columnwidth}@{}}{``The reader can adjust the radius of a circle using a slider, and as the radius changes, the visualization updates the circle while recalculating and displaying the circumference, diameter, and ratio, allowing the reader to see that the ratio stays roughly the same.''} \\
\midrule
\multicolumn{2}{@{}l}{\textbf{SRTC Interaction Specification}} \\
\midrule
\textbf{S} & \texttt{r}: slider $[0.5, 5]$, default 1; \texttt{C}: derived $2\pi r$; \texttt{D}: derived $2r$; \texttt{ratio}: derived $C/D$ \\
\textbf{R} & A circle whose size reflects $r$; labels showing $C$, $D$, and ratio \\
\textbf{T} & Dragging the slider changes $r$; $C$, $D$, ratio update automatically \\
\textbf{C} & ratio $\approx 3.14159$ regardless of $r$ \\
\bottomrule
  \end{tabularx}
\end{table}


==> sec/ui.tex <==


\begin{figure*}[htbp]
  \centering
  \includegraphics[width=0.85\linewidth]{image/table3_grouped_bars}

  \caption{Automated evaluation results for \system vs.\ three multi-agent baselines across three backbone LLMs.
    Content Richness (CR) and Interaction Quality (IQ) are normalized to $[0,1]$.
    Interaction Functionality is on a 0--1 scale; Efficiency is measured in characters per second (chars/s).}
  \label{fig:auto_eval}
  \vspace{-1em}
\end{figure*}

\section{User Interface}
\label{sec:ui}

Figure~\ref{fig:system} shows the \system user interface, which consists of three panels: a sidebar (A), a center panel (B), and an AI assistant panel (C). The sidebar (A) provides a ``New Doc'' button (A1) to start a new generation and a history list (A2) of previously generated documents. The center panel (B) guides users through a four-stage workflow indicated by the top navigation bar (B1): Topic, Spec, Style, and Doc. A download button (B2) allows exporting the final document. The AI assistant panel (C) provides a chat interface (C1) for refining the spec or the generated document through natural language conversation.

\paragraph{Stage 1: Topic.} The user enters a topic of interest in the input field (B3) and clicks ``Generate Spec'' to start the pipeline.

\paragraph{Stage 2: Spec.} The Planner generates a DocSpec, displayed as a list of knowledge units (Figure \ref{fig:system}b). Each unit shows its title, text description, and SRTC Interaction Specification. Users can edit, reorder, add, or delete knowledge units before proceeding.

\paragraph{Stage 3: Style.} The Styler generates a Style Palette with two columns: Writing Style and Interaction Style (Figure \ref{fig:system}c). Each column contains several dimensions with LLM-generated options. Users can select an option, choose ``Auto'' to let the LLM decide, or provide custom instructions.

\paragraph{Stage 4: Doc.} The Executor generates the final interactive document, rendered in the center panel (Figure \ref{fig:system}d). Users can interact with and download the document. The chat assistant (C1) allows further refinement through natural language requests.



